Formalizing Piecewise Affine Activation Functions of Neural Networks in Coq

Verification of neural networks relies on activation functions being piecewise affine (pwa) -- enabling an encoding of the verification problem for theorem provers. In this paper, we present the first formalization of pwa activation functions for an interactive theorem prover tailored to verifying neural networks within Coq using the library Coquelicot for real analysis. As a proof-of-concept, we construct the popular pwa activation function ReLU. We integrate our formalization into a Coq model of neural networks, and devise a verified transformation from a neural network N to a pwa function representing N by composing pwa functions that we construct for each layer. This representation enables encodings for proof automation, e.g. Coq's tactic lra -- a decision procedure for linear real arithmetic. Further, our formalization paves the way for integrating Coq in frameworks of neural network verification as a fallback prover when automated proving fails.

==> sections/related-work.tex <==
\section{Related Work}
\label{s:related-work}
%short & broad
most deductive verification approaches based on piecewise affine activation functions.
few approaches for interactive theorem provers.

%machine learning in Coq
paper from which we adapted the model is about ...
while they consider ReLU -- a piecewise affine activation function, 
they do not lay a foundation for PAF. 
To the best of our knowledge, first formalization in any interactive theorem prover.
